Rainbow numbers for $x_1+x_2=kx_3$ in $\mathbb{Z}_n$

In this work, we investigate the fewest number of colors needed to guarantee a rainbow solution to the equation $x_1 + x_2 = k x_3$ in $\mathbb{Z}_n$. This value is called the Rainbow number and is denoted by $rb(\mathbb{Z}_n, k)$ for positive integer values of $n$ and $k$. We find that $rb(\mathbb{Z}_p, 1) = 4$ for all primes greater than $3$ and that $rb(\mathbb{Z}_n, 1)$ can be deterimined from the prime factorization of $n$. Furthermore, when $k$ is prime, $rb(\mathbb{Z}_n, k)$ can be determined from the prime factorization of $n$.

==> GenIntro.tex <==
In this section, we move away from the Schur equation and aim to prove similar results with the equation's constant generalized to an arbitrary integer.
We mostly focus on $k$ being prime, which we denote as $p$, but some of our results hold when $k$ is composite.

In Section \ref{SectionGenKPrimes}, we detail our results on colorings of cyclic groups whose order is prime.
Then we produce a recursive formula to calculate $rb(\mathbb{Z}_n,p)$ by producing a tight lower bound in Section \ref{SectionGenKLowerBound} and a tight upper bound in Section \ref{SectionGenKUpperBound}

==> GenPrimes.tex <==
Many of our results in this section are derived from the implications of Llano and Montejano \cite{LM} Theorem 2, which we state here:

\begin{theorem}\label{3ColorPrimes}[\cite{LM}, Theorem 2]
A 3-coloring $\mathbb{Z}_p = A \cup B \cup C$ with $1 \leq |A| \leq |B| \leq |C|$ is rainbow-free for $x + y = cz$ if and only if, up to dilation, one of the following holds.

\begin{enumerate}
\item $A = \{0\}$ and both $B$ and $C$ are symmetric and $\langle c \rangle$-periodic subsets.
\item $A = \{1\}$ for 
\begin{itemize}
\item [(i)] $c=2$, $(B-1)$ and $(C-1)$ are symmetric and $\langle 2 \rangle$-periodic subsets.
\item [(ii)] $c = -1$, $(B\setminus \lbrace 2 \rbrace ) + 2^{-1}$, $(C\setminus \lbrace 2 \rbrace) + 2^{-1}$ are symmetric subsets.
\end{itemize}
\item $|A| \geq 2 $, for $c = -1$ and $A,B,$ and $C$ are arithmetic progressions with difference 1 such that $A = \lbrack a_1, a_2 - 1 \rbrack$, $B = \lbrack a_2, a_3 - 1 \rbrack$, and $C = \lbrack a_3, a_1 - 1 \rbrack$, with $(a_1 + a_2 + a_3) = 1$  or $2$.
\end{enumerate}
\end{theorem}

Since we are generally more concerned with the existence of rainbow-free colorings where 0 is uniquely colored, we are able to derive the following corollary from Theorem \ref{3ColorPrimes}.

\begin{cor}\label{0unique}
When $k \not \equiv 0 \mod p$, $\mathbb{Z}_p$ has a rainbow-free 3-coloring for $x_1+x_2=kx_3$ if and only if it has a rainbow-free 3-coloring such that 0 is uniquely colored, and the other two colors are symmetric and $\langle k\rangle$-periodic subsets, i.e., a coloring that falls into Case (1) of Theorem \ref{3ColorPrimes}.
\end{cor}
\begin{proof}
If $k \not \equiv -1 \mod p$ and $k \not \equiv 2 \mod p$, then a rainbow-free 3-coloring can only fall into case (1) of Theorem \ref{3ColorPrimes}, so if there is a rainbow-free 3-coloring, it must be of this form.


If $k \equiv -1 \mod p$, all $\langle k\rangle$-periodic subsets consist of just the elements at position $-x \mod p$ and $x \mod p$, which are symmetric subsets. Thus, $\mathbb{Z}^*_p$ can be split into any two subsets which are symmetric and consequently $\langle k \rangle$-periodic, as long as $p\geq5$. 
Thus, $\mathbb{Z}_p$, $p\geq5$, can always be colored with 3-colors in the form described in case (1), except when $p=3$. However, there is no way to 3-color $p=3$ without a rainbow triple for any $k$, as $(1,-1,0)$ is a triple for all $k$.

If $k \equiv 2 \mod p$, a 3-coloring in the form stated in case (2)(i) does not have 0 uniquely colored, but some element $s\in\mathbb{N}, 1\leq s \leq p-1$ is uniquely colored.
For any triple $(x_1,x_2,x_3)$ in $\mathbb{Z}_p$, $(x_1-s,x_2-s,x_3-s)$ is also a triple, because if
$$x_1+x_2\equiv k x_3\mod p$$
then,
$$x_1+x_2-2s\equiv k x_3-ks \equiv kx_3-2s \mod p.$$
If coloring $c$ is a rainbow-free coloring of $\mathbb{Z}_p$ where $k \equiv 2 \mod p$, and 0 is not uniquely colored, take the dilation where 1 is uniquely colored.
Then, $\hat{c}(x):=c(x+1)$ is also a rainbow-free coloring. 
Therefore, if we have a rainbow-free coloring as in case (2)(i), we can shift every element of the coloring by $1$ and create a rainbow-free coloring $\hat{c}(x):=c(x+1)$, where 0 is uniquely colored and $B$ and $C$ are symmetric.
\end{proof}

We also used the above results to explicitly state when a prime is not 3-colorable, i.e., when $rb(\mathbb{Z}_p, k)=3$. 

\begin{cor}
When $k \not \equiv 0 \mod p$, $rb(\mathbb{Z}_p, k)=3$ if and only if $\langle k \rangle$ is a multiplicative generator for all of $\mathbb{Z}^*_p$ or $\langle k \rangle$ is a multiplicative generator for half of $\mathbb{Z}^*_p$ and $\langle -k \rangle$ is a multiplicative generator for the other half of $\mathbb{Z}^*_p$.
\end{cor}

\begin{proof}
By Corollary \ref{0unique}, we know that $\mathbb{Z}_p$ has a rainbow-free 3-coloring for $x_1+x_2=kx_3$ if and only if it has a rainbow-free 3-coloring such that 0 is uniquely colored and the other two colors are symmetric and in $\langle k\rangle$ periodic subsets.
If $\langle k\rangle$ generates the entirety of $\mathbb{Z}^*_p$, there is no way to create two color classes that are both $\langle k\rangle$ periodic, and thus $\mathbb{Z}_p$ cannot be 3-colored.
If $\langle k\rangle$ generates only half of $\mathbb{Z}^*_p$, and $\langle -k\rangle$ generates the other half of $\mathbb{Z}^*_p$, all elements of $\mathbb{Z}^*_p$ would again necessarily be in the same color class, and so $\mathbb{Z}_p$ is not 3-colorable. 

Otherwise, let $A=\{0\}$, let $B=\{e|e\in\langle k\rangle\}\cup\{e|e\in\langle -k\rangle\}$, and let $C=\mathbb{Z}^*_p\setminus B$. 
Then, $B$ and $C$ are both symmetric and $\langle k\rangle$ periodic subsets, and $A=\{0\}$.
$A\cup B\cup C=\mathbb{Z}_p$ and is a rainbow-free coloring of $\mathbb{Z}_p$. Thus, $rb(\mathbb{Z}_p, k)\geq 3$.
\end{proof} 

With these two results, we begin to prove an upper bound on $rb(\mathbb{Z}_p,k)$ when we know $rb(\mathbb{Z}_p,k) \geq 3$. First, we prove the following structural lemma.

\begin{lemma}\label{No3Singleton}
Let $q$ be prime, and let $k$ be an integer relatively prime to $q$.
In a rainbow-free $r$-coloring of $\mathbb{Z}_q$ with $r>3$, three color classes cannot be singleton.
\end{lemma}
\begin{proof}
Assume for the sake of contradiction we have a rainbow-free $r$-coloring of $\mathbb{Z}_q$ with $r>3$ in which three color classes are singleton.
Thus, let $u_1$, $u_2$, and $u_3$ be three distinct integers in $\mathbb{Z}_q$ which are uniquely colored.
Because $k$ and $q$ are relatively prime we have the following triples:
\begin{align}
& u_1 + u_2  \equiv  k \cdot u_a \mod q & a \in \{1,2\} & \\
& u_1 + u_3  \equiv  k \cdot u_b \mod q & b \in \{1,3\} & \\
& u_2 + u_3  \equiv  k \cdot u_c \mod q & c \in \{2,3\} & 
\end{align}
Additionally, we know that $\{a,b,c\} = \{1,2,3\}$ because $k$ and $q$ are relatively prime. Without loss of generality we choose $a=1$, $b=3$, $c=2$. 
Then we add equations (1), (2), and (3) to get
$$ 2u_1 + 2u_2 + 2u_3 \equiv k(u_1 + u_2 + u_3) \mod q.$$
This implies that $k \equiv 2 \mod q$.
Now, adding equations (1) and (2) yields
$$ 2u_1 + u_2 + u_3 \equiv k(u_1 + u_3) \mod q.$$
Since $k \equiv 2 \mod q$ we get
$$ 2u_1 + u_2 + u_3 \equiv 2u_1 + 2u_3 \mod q.$$
This implies that $u_2 \equiv u_3 \mod q$, which is a contradiction.
\end{proof}

Following from this lemma and case (1) and (2)(i) of Theorem \ref{3ColorPrimes}, we are able to prove $rb(\mathbb{Z}_1, k)\leq 4$ for all $k \not \equiv -1 \mod q$, $k \neq q$.

\begin{prop}\label{PrimeKNot-1}
Let $q$ be prime and let $k$ be an integer relatively prime to $q$ such that $k \not \equiv -1 \mod q$.
Let $c$ be an $r$-coloring of $\mathbb{Z}_q$ with $r \geq 4$.
Then $c$ contains a rainbow triple.
Consequently, $rb(\mathbb{Z}_q,p) \leq 4$.
\end{prop}
\begin{proof}
From Lemma \ref{No3Singleton}, $c$ has at most two singleton color classes.
If $c$ has two singleton color classes, then without loss of generality, let $R$ and $G$ be these color classes.
If $c$ has one singleton color class, without loss of generality, let $R$ be this singleton color class and let $G$ be another non-singleton color class.
Lastly, if $c$ has no singleton color classes, then let $R$ and $G$ be any distinct color classes of $c$.
Regardless of which case we are in, define $\hat{c}$ to be a 3-coloring whose color classes are the union of color classes of $c$, one of which being $R \cup G$.
Notice that this construction ensures that $\hat{c}$ does not have any singleton color classes.
Since $k \not \equiv -1 \mod q$, then our 3-coloring $\hat{c}$ must fall into case 1 or 2 of Theorem \ref{3ColorPrimes}.
But both cases require that $\hat{c}$ has at least one singleton color class.
Thus, by this theorem, $\hat{c}$ is not rainbow-free which implies that $c$ contains a rainbow triple.
\end{proof}

This shows that for cases where $k \not \equiv -1 \mod q$, $k \neq q$ $rb(\mathbb{Z}_q,p) = 3 \textrm{ or } 4$. 
To expand our results to all $k \neq q$, we first use Theorem \ref{3ColorPrimes} to obtain the following property of colorings with all color classes of cardinality greater than 1 and $k \equiv -1 \mod q$.

\begin{cor}\label{APcor}
Let $c$ be a 3-coloring of $\mathbb{Z}_q$ such that it falls into case (3) of Theorem \ref{3ColorPrimes}.
Then, in any dilation of $c$, the color classes $A$, $B$, and $C$ are arithmetic progressions with the same difference $d$. 
\end{cor}

\begin{proof}
Rainbow-free colorings are invariant up to dilation. 
Thus, no matter what dilation of $c$ we take, there is a dilation which can form a coloring where each color class $A$, $B$, and $C$ are arithmetic progressions with difference one.
The reverse is also true, that any dilation of $c$ is a dilation of the coloring where each color class $A$, $B$, and $C$ are arithmetic progressions with difference one.
Therefore, $c$ is equivalent to $aA\cup aB \cup aC$ for some $a \in \mathbb{Z}^*_q$.
Hence, $c$ is made up of arithmetic progressions with difference $a$, and all dilations of $c$ have three color classes which are each arithmetic progressions with difference $d \in \mathbb{Z}^*_q$.
\end{proof}

Let $A = \{a+i \cdot d_a | 0 \leq i \leq n\}$ and $B = \{b+i \cdot d_b | 0 \leq i \leq m\}$ be two arithmetic progressions.
Then we have the following two definitions.
$A$ and $B$ are said to be \textit{stacked} if and only if $d_a = d_b$ and either $b = a + (n+1) d_a$ or $a = b + (m+1) d_b$.
$A$ and $B$ are said to be \textit{shuffled} if and only if $d_a = d_b$, $b = a + d_a/2$, and $b + m \cdot d_b = a + n \cdot d_a \pm d_a/2$.


\begin{lemma}\label{APs}
Let $\mathbb{Z}_n$ be partitioned into set $X_1$, $X_2$, $X_3$, and $X_4$ for some integer $k \geq 4$, and let $A = X_i \cup X_j$, $B = X_k$, and $C = X_l$ for $\{i,j,k,l\}=\{1,2,3,4\}$.
If $A$, $B$, and $C$ are all arithmetic progressions for any selection of $i$, $j$, $k$, and $l$, then $X_t$ for $t \in \{1,2,3,4\}$ are all arithmetic progressions with distance $d$.
\end{lemma}
\begin{proof}
Assume for the sake of contradiction that there exists an $a \in \{1,2,3,4\}$ such that $X_a$ is not an arithmetic progression.
Thus, if we let $B = X_a$, then $B$ is not an arithmetic progression, which shows that if $A$, $B$, and $C$ are all arithmetic progressions for any selection of $i$, $j$, $k$, and $l$, then $X_t$ for $t \in \{1,2,3,4\}$ are all arithmetic progressions.
%Notice that the only way for two arithmetic progressions, say $X_1$ and $X_2$, with different differences to be combined into one arithmetic progression is if, without loss of generality,
\end{proof}

Finally, we combine these results to show that $rb(\mathbb{Z}_q, p)\leq4$ when $k \equiv -1 \mod p$. 

\begin{prop}\label{PrimeK=-1}
Let $q>2$ be prime and let $k\in\mathbb{N}$ such that $k\equiv -1 \mod q$. 
Let $c$ be an $r$-coloring of $\mathbb{Z}_q$, with $r\geq 4$. 
Then $c$ contains a rainbow triple.
\end{prop}
\begin{proof}
Since $k\equiv -1 \mod q$, $q$ and $k$ are relatively prime. 
Therefore by Lemma \ref{No3Singleton}, there cannot be three singleton color classes in $c$. We now look at three cases, where $c$ has two, one, and zero singleton color classes.

Let $c$ be an $r$-coloring of $\mathbb{Z}_q$, $r\geq 4$ with two singleton color classes, and without loss of generality let these two singleton color classes be $R$ and $B$. 
Define $\hat{c}$ to be a 3-coloring $C_1\cup C_2 \cup C_3=\mathbb{Z}_q$ such that each $C_i$ is the union of color classes in $c$. Take $C_1=R$, $C_2=G$ and $C_3$ equal to the union of all other color classes in $c$.
Since $\hat{c}$ has a singleton color class, this coloring falls into either case (1) or case (2)(ii) of Theorem \ref{3ColorPrimes}. 
In either case, only one of $R$ and $B$ can be the color $A$, and the other must be symmetric.
\textbf{}
Since $q$ is prime, it is odd, and $q-1$ being symmetric requires the color classes in it to be even.
Whichever of $R$ and $B$ is not the color $A$ is odd, and therefore cannot be symmetric.
Thus, any $r$-coloring of $\mathbb{Z}_q$ with $r\geq 4$ two singleton color classes contains a rainbow triple.

Let $c$ be an $r$-coloring of $\mathbb{Z}_q$ with $r\geq4$ and one singleton color class. Without loss of generality let this color class  be $R$.
% Let two of the other $r-1$ color classes be $B$ and $G$.
% Define $\bar{c}$ to be a 4-coloring $R\cup B \cup G \cup Y=\mathbb{Z}_q$
Define $\hat{c}$ to be a 3-coloring of $\mathbb{Z}_q$ such that the color-classes of $\hat{c}$ are unions of the color classes of $c$ and whichever color class $R$ is in in $\hat{c}$ is the union of at least two color classes. 
Taking the union of $R$ with any of the other color classes will result in a coloring $\hat{c}$ where each color class has a cardinality of at least 2. 
Thus, our coloring $\hat{c}$ must fall into case (3) of Theorem \ref{3ColorPrimes}. 

In $c$, the number that is colored $R$ is either adjacent to 2 different colors, or is adjacent to the same color on either side.
Examine the case where $R$ is adjacent to 2 different colors, and denote the color class coloring the position to the left of $R$ as $G$ and the color class coloring the position to the right of $R$ as $B$. 
Then, there is some 3-element string where we have the pattern $GRB$.
To create our coloring $\hat{c}$, first take the union $R\cup G$. 
By Corollary \ref{APcor}, a coloring of $\mathbb{Z}_q$ with color classes all having cardinality $\geq 2$ is rainbow-free if and only if all of three color classes are arithmetic progressions.
If $R \cup G$ is not an arithmetic progression, then $\hat{c}$ has a rainbow.
If $R \cup G$ is an arithmetic progression, then it must have difference 1. 
Similarly if $R \cup B$ is not an arithmetic progression, $\hat{c}$ has a rainbow, and if $R \cup B$ is an arithmetic progression, it must have difference 1.
Define $Y$ to be the union of all color classes in $c$ other than $R$, $G$, and $B$.
By Lemma \ref{APcor}, $Y$ must also be a arithmetic progression with difference 1.
Therefore, $R \cup Y$ is not an arithmetic progression, as the number colored $R$ must have a difference greater than 2 from the nearest element of Y, and $\hat{c}$ must contain a rainbow triple.

Next, look at the case where $R$ is adjacent to the same color on either side, and without loss of generality let this color be $B$. 
If all color classes other than $R$ and $B$ are arithmetic progressions with difference 1, take the union of $R$ with any of these color classes in $\hat{c}$.
This color class will not be an arithmetic progression, and thus $\hat{c}$ contains a rainbow triple.
If at least one of the color classes other than $R$ and $B$ is not an arithmetic progression with difference 1, take $R\cup B$ as a color class in $\hat{c}$, let another color class in $\hat{c}$ be equal to one of the color classes that is not an arithmetic progression with difference 1, and let the third color class in $\hat{c}$ be the union of all other color classes in $c$. 
Then, either $R\cup B$ is an arithmetic progression with difference 1, in which case not all three color classes in $\hat{c}$ have the same difference, so $\hat{c}$ must contain a rainbow triple, or, $R\cup B$ is not an arithmetic progression and $\hat{c}$ has a rainbow triple. 

Let $c$ be a 4-coloring of $\mathbb{Z}_q$ with no singleton color classes.
Notice that if the color classes of $c$ are not as described in Lemma \ref{APs}, then a 3-coloring could easily be created from the union of the color classes in $c$ such that at least one color class is not an arithmetic progression.
In this case, the 3-coloring created would not fall into case (3) of Theorem \ref{3ColorPrimes}.
Also, it could not fall into case (1) or (2), as no color classes are singleton.
Therefore, $c$ would not be rainbow-free, so let us assume that every color class is an arithmetic progression with the same distance $d$.
Now, without loss of generality, take the color class $R$.
By Lemma \ref{APs}, we know that the other three color classes will be arranged such that one is stacked to the right, one is stacked to the left, and one is shuffled.
Without loss of generality, let these color classes be $B$, $G$, and $Y$, respectively.
Now create $\hat{c}$, a 3-coloring of $\mathbb{Z}_q$ from $c$ such that one color class is the union of $R$ and $Y$.
Because $R$ and $Y$ were shuffled, and the distance between the first and second elements in both $R$ and $Y$ is $d$, then $R \cup Y$ is an arithmetic progression of distance $d/2$.
Because no color classes in $c$ were singleton, then $\hat{c}$ cannot fall into case (1) or (2) of Theorem \ref{3ColorPrimes}.
Additionally, the three color classes in $\hat{c}$ will be arithmetic progressions with distances of either $d$ or $d/2$.
Because not all three have identical distances, $\hat{c}$ cannot be dilated to produce 3 arithmetic progression color classes of distance 1, so $\hat{c}$ cannot fall into case (3) of Theorem \ref{3ColorPrimes}.
Thus, $\hat{c}$ must not be rainbow-free, implying that $c$ is not rainbow-free.

Note that the argument above shows that any 4-coloring of $\mathbb{Z}_q$ is not rainbow-free, which immediately shows that any $r$-coloring of $\mathbb{Z}_q$ with $r \geq 4$ contains a rainbow triple.
\end{proof}

Note that since $rb(\mathbb{Z}_p, k)$ is always 3-colorable when $p\geq5$ and $k\equiv-1\mod p$, $rb(\mathbb{Z}_p, k)=4$ in these cases. Our final result on $rb(\mathbb{Z}_p, k)$ is for the case when $k=p$, i.e., $rb(\mathbb{Z}_p, p)$.

\begin{prop}\label{PrimeK=P}
Let $p \geq 3$ be prime and let $k = p$. 
Then, $rb(\mathbb{Z}_p, p) =\frac{p+1}{2}+1$.
\end{prop}

\begin{proof}
Since $k=p$, all triples are in the form $(x, -x, y)$, where $x \neq -x, y$, $-x \neq y$. 
Therefore, if we place color $R$ only on position 0, i.e. $R=\{0\}$, and create color classes $C_i=\{i, -i\}$ for $1\leq i \leq \frac{p-1}{2}$, then all triples have two members in one color class and we have used $\frac{p+1}{2}$ colors. 
Thus, $rb(p) \geq \frac{p+1}{2}+1$.

Next, color $p$ with $\frac{p+1}{2}+1$ colors. 
By the pigeon hole principle, there must be at least two singleton color classes, and at least one of these singleton color classes is not the color of $0$. 
Therefore, there must be some symmetric pair, $(x, -x)$, $x \neq -x$, which is colored with two different colors. 
Additionally, $\frac{p+1}{2}+1\geq 3$ for $p\geq3$, so there must be at least one element $y$, different from $x$ and $-x$, which is colored with a third color. 
The pair $(x, -x)$ creates a triple with any $y \neq x$, $y \neq -x$ in the form $(x, -x, y)$, and thus we have a rainbow triple. 
Therefore, $rb(p) = \frac{p+1}{2}+1$ when $k=p$.
\end{proof}

Notice then, that Theorem \ref{GenKPrimeValues} is established by Propositions \ref{PrimeKNot-1}, \ref{PrimeK=-1}, and \ref{PrimeK=P}.
